A High-Level LTL Synthesis Format: TLSF v1.1

We present the Temporal Logic Synthesis Format (TLSF), a high-level format to describe synthesis problems via Linear Temporal Logic (LTL). The format builds upon standard LTL, but additionally allows to use high-level constructs, such as sets and functions, to provide a compact and human-readable representation. Furthermore, the format allows to identify parameters of a specification such that a single description can be used to define a family of problems. Additionally, we present a tool to automatically translate the format into plain LTL, which then can be used for synthesis by a solver. The tool also allows to adjust parameters of the specification and to apply standard transformations on the resulting formula.

==> eptcsdata.tex <==
\providecommand{\firstpage}{112}
\providecommand{\publicationstatus}{Dimitrova, Piskac (Eds.): Fifth Workshop on\\ 
Synthesis (SYNT 2016)\\
EPTCS 229, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.229.10}{10.4204/EPTCS.229.10}}
\usepackage{ifthen}
\providecommand{\eptcs}{{\sl Electronic Proceedings in Theoretical Computer Science}}
\providecommand{\opa}{, Open Publishing Association}
\providecommand{\finishreference}[6]{#1 #2#3, pp. #4--#5, \doi{10.4204/EPTCS.#2.#6}}
\providecommand{\thisvolume}[2][\eptcs]{%
 \ifthenelse{\equal{#2}{5}}{\finishreference{#1}{229}{\opa}{133}{148}{11}}{%
 \ifthenelse{\equal{#2}{13}}{\finishreference{#1}{229}{\opa}{149}{177}{12}}{%
 this volume of #1\opa}}}

